Current validation practice undermines surgical AI development

Surgical data science (SDS) is rapidly advancing, yet clinical adoption of artificial intelligence (AI) in surgery remains limited, with inadequate validation as an important contributing factor. Existing validation practices often neglect the temporal and hierarchical structure of intraoperative videos, yielding misleading or clinically irrelevant results. We introduce a comprehensive catalogue of validation pitfalls in AI-based surgical video analysis, derived from a multi-stage Delphi process with 92 international experts. Pitfalls span three categories: (1) data, (2) metric selection/configuration, and (3) aggregation and reporting. A systematic review of surgical AI papers reveals that these pitfalls are widespread. Experiments on surgical video datasets show that ignoring temporal and hierarchical data structures can understate uncertainty, obscure critical failure modes, and alter algorithm rankings. To address these shortcomings, we provide consensus-based best practices compiled. Together, this work provides an evidence-based framework for rigorous validation of surgical video analysis algorithms, guiding benchmarking, reporting, regulatory review, and clinical translation.

==> extended-data.tex <==
\ExtendedDataFiguresOn
\setcounter{figure}{0}
\section{Extended Data}
\label{sec:extended-data}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/ED-Fig1.pdf}
    \caption{\textbf{P1.1 -- Non-representativeness, low quality, and low relevance of data. }(a) Example of excluding low-quality frames during model development, which can lead to overestimation of algorithm robustness and limited generalization in real-world settings. In this example, algorithms trained on data with such frames omitted perform considerably worse regarding their Dice similarity coefficient (DSC) when tested on data containing challenging conditions (results based on data from the Robust Medical Instrument Segmentation (RobustMIS) challenge 2019 \cite{ross2021comparative}). In this case, the performance gap even leads to changes in the relative ranking of algorithms. Mean DSC scores are color-coded (green: high scores; orange: low scores). (b) Example of geographical imbalance of data, highlighting limited representativeness of surgical data science (SDS) datasets. The map shows the geographical distribution of the datasets used in biomedical image analysis challenges involving surgical or endoscopic data conducted between 2018 and 2023 (n = 65 tasks across 14 challenges). Most data originate from a few Western European countries, particularly France, the United Kingdom, and Germany, whereas large parts of the world remain unrepresented.}
    \label{fig:extended-fig1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/ED-Fig2.pdf}
    \caption{\textbf{P1.2 -- Limited sample size/test cohorts, or data imbalance.} The figure demonstrates the impact of class imbalance and limited test set size on performance stability for the task of surgical action triplet recognition in cholecystectomy (here: CholecT45 \cite{nwoye2023cholectriplet2021}). (a) The distribution of triplet classes across five randomly selected videos, sorted by the total number of occurrences per class (here: top 15 triplet classes), is highly imbalanced, with some classes frequent and many rare or absent, highlighting the risk of inconsistent class coverage. (b) To reflect the data split of CholecT45 (nine videos per fold), we randomly sampled nine videos for 30 runs. In each run, a swin-based transformer model trained on the original CholecT45 training data with multi-task learning and soft labels derived via a multi-teacher strategy was validated on the sampled videos \cite{yamlahi2023self}. The boxplots show high variability in per-video mean Average Precision (mAP) across runs, demonstrating the unstable and unreliable nature of class-averaged metrics such as mAP under the joint influence of limited test cohort size and heterogeneous class coverage.}
    \label{fig:extended-fig2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/ED-Fig3.pdf}
    \caption{\small\textbf{(a) P1.3 -- Existence of spurious correlations within data.} In this example, a bleeding detection algorithm is trained on a biased development dataset where suction/irrigation devices are only present during bleeding. As a result, the algorithm mistakenly learns to associate the presence of these tools with bleeding events, rather than detecting blood itself. During deployment, the algorithm fails when suction is used outside of bleeding contexts or when blood appears without suction. This illustrates how spurious correlations in biased datasets can undermine clinically important tasks such as bleeding detection. \textbf{(b) P1.4 -- Incomplete annotation or missing contextual information.} Validation may be compromised, especially in safety-critical surgical phases, if annotations are incomplete or lack contextual detail needed to assess model performance. (1) Annotation completeness refers to the extent to which all relevant phases, events, or entities are labeled in sufficient detail for the intended task, but does not necessarily align with clinical relevance: In this example, the Clipping Cutting phase, despite being highly safety-relevant, is poorly annotated, limiting robust validation. In contrast, longer and less critical phases are better annotated, skewing performance estimates. Phase duration is represented by bubble size. (2) Even when frames are annotated, missing contextual information such as anatomical region or metadata can compromise interpretability and validity. In this example, the same surgical frame (from CholecT45 \cite{nwoye2023cholectriplet2021}) is annotated minimally (top; phases only), while the bottom row illustrates a context-aware annotation including semantic and procedural details enabling more meaningful and clinically robust validation.}
    \label{fig:extended-fig3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/ED-Fig4.pdf}
    \caption{\textbf{P1.6 -- Poor data splitting.} In this example, a random split of frames across training and test sets over all patients leads to data leakage, as images from the same patient appear in both sets. This results in overly optimistic performance on the development test data (Dice similarity coefficient (DSC) of 0.74) but substantially lower performance on unseen deployment data (DSC = 0.55). Results are based on the Robust Medical Instrument Segmentation (RobustMIS) challenge 2019 \cite{ross2021comparative} binary segmentation data and and a U-Net implementation, comparing training where frames from every patient are split 60/20/20 training/validation/testing with training where patients are used wholly for training, validation, or testing in a 60/20/20 split.}
    \label{fig:extended-fig4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/ED-Fig5.pdf}
    \caption{\textbf{P2.1 -- Mismatch of metrics and clinical needs.} Despite both algorithms achieving the same Dice similarity coefficient (DSC = 0.82), \textit{Algorithm 1} accurately captures the gallbladder’s outline, while \textit{Algorithm 2} produces a poorly shaped segmentation. The Normalized surface distance (NSD) better reflects the clinically relevant boundary accuracy required for this use case. Images from CholecSeg8k \cite{hong2020cholecseg8k}. Note: In clinical practice, certain boundaries (e.g., gallbladder-liver interface) may be more critical than others -- a nuance which is captured by neither DSC nor NSD.}
    \label{fig:extended-fig5}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/ED-Fig6.pdf}
    \caption{\textbf{P2.3 -- Lack of handling of video annotation uncertainties. }In this example, inconsistencies between expert raters (a) in phase annotations occur at transition points and (b) in instrument segmentation masks. These areas of uncertainty lead to changes in performance scores (here: Accuracy and Dice similarity coefficient (DSC)) depending on which expert is considered as the reference. DSC values were computed for the full image, not the zoomed region. Images and annotations in (b) are from inter-rater variability analysis of the Robust Medical Instrument Segmentation (RobustMIS) challenge \cite{ross2021comparative}.}
    \label{fig:extended-fig6}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figs/ED-Fig7.pdf}
    \caption{\textbf{P2.4 -- Lack of robustness of metrics across varying real-world conditions (here: image resolution (a) and frame rate (b)).} In this example, a fixed classifier (ResNet50) is validated on surgical video data (Cholec80 \cite{twinanda2016endonet}) under varying real-world conditions: (a) Different spatial resolutions (100\%, 75\%, 50\%) and (b) sampled at 1, 3, and 5 frames per second (FPS), simulating typical variability in real-world acquisition or compression conditions. Despite using identical model weights and validating on the same underlying procedure, performance metrics (here: Accuracy, Positive predictive value (PPV), Recall, F1-score) vary noticeably with resolution and frame rate. These variations arise not from changes in the model or task, but from the metric's sensitivity to input resolution, illustrating a lack of robustness in metrics under plausible real-world conditions. }
    \label{fig:extended-fig7}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/ED-Fig8.pdf}
    \caption{\textbf{(a) P2.5 -- Non-standardized configuration and definition of metrics. }In this example, relaxed metrics, which allow for a less strict definition of True Positives (TPs), are applied in phase transition areas where expert annotations often show inconsistencies. The non-relaxed macro scores, i.e., unweighted mean across classes, are compared to four different variants of relaxed metrics (application-dependent (AD) scores, relaxed metrics for the Cholec80 dataset, and two corrected versions v1 (cutting values at 1.00) and v2 (adapting the denominator of the definition); see \cite{funke2023metrics}), resulting in substantial differences in Sensitivity and Positive predictive value (PPV) values. \textbf{(b) P2.6 -- Non-suitability of hyperparameters from unrelated domains.} The choice of detection thresholds (here: Intersection over Union (IoU)) critically impacts the reported detection performance (here: polyp detection during capsule endoscopy). This example compares a clinical threshold configuration (blue box; Average Precision (AP)[0.05:0.50]) and a standard machine learning (ML) configuration (orange box; AP[0.50:0.95]) on the same images. The stricter ML configuration penalizes several detections as False Positives (FP) that would be acceptable in a clinical setting (True Positives (TP)), leading to a much lower overall AP. Note that the phrasing "for most IoU thresholds" refers to a detection being counted as a TP/FP across the majority of thresholds used in the AP calculation.}
    \label{fig:extended-fig8}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/ED-Fig9.pdf}
    \caption{\textbf{(a) P3.3 -- Lack of contextualization of performance values.} In this example, the specific clinical use case prioritizes high Sensitivity, as missing a positive event could have severe consequences. Here, algorithm A3 is ranked highest based on Accuracy but fails to meet the required clinical Sensitivity threshold ($\geq$ 95\%). The lack of contextualization of the performance values conceals the fact that none of the models meet both clinical thresholds. \textbf{(b) P3.4 -- Lack of uncertainty handling.} Performance rankings based solely on point estimates can be misleading without reporting uncertainty. In this example, algorithm A1 is considered the best due to its highest mean Dice similarity coefficient (DSC) score. However, confidence intervals (CIs) of the pairwise differences show that for several competitors there is no clear evidence that A1 outperforms them, since the CIs include 0. Circles indicate mean differences, and vertical lines show the hierarchical bootstrap CI (see Methods for details) of differences. Results are based on RobustMIS 2019 \cite{ross2021comparative} binary segmentation top 6 algorithms.}
    \label{fig:extended-fig9}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figs/ED-Fig10.pdf}
    \caption{Scatterplot of used metrics in the 2023 Medical Image Computing and Computer Assisted Intervention (MICCAI) conference surgical data science (SDS) papers. Here, the metrics are shown for various SDS tasks. Both tasks and metrics are sorted by frequency of usage (metrics: top to bottom; tasks: left to right). The size of the blobs corresponds to the frequency of metric occurrence. According to the screening, only a single paper reported a temporal metric, the Consistency Score (green).}
    \label{fig:extended-fig10}
\end{figure}


\ExtendedDataFiguresOff
